A Game-Theoretic Approach to Multi-Objective Resource Sharing and Allocation in Mobile Edge Clouds

Mobile edge computing seeks to provide resources to different delay-sensitive applications. However, allocating the limited edge resources to a number of applications is a challenging problem. To alleviate the resource scarcity problem, we propose sharing of resources among multiple edge computing service providers where each service provider has a particular utility to optimize. We model the resource allocation and sharing problem as a multi-objective optimization problem and present a \emph{Cooperative Game Theory} (CGT) based framework, where each edge service provider first satisfies its native applications and then shares its remaining resources (if available) with users of other providers. Furthermore, we propose an $\mathcal{O}(N)$ algorithm that provides allocation decisions from the \emph{core}, hence the obtained allocations are \emph{Pareto} optimal and the grand coalition of all the service providers is stable. Experimental results show that our proposed resource allocation and sharing framework improves the utility of all the service providers compared with the case where the service providers are working alone (no resource sharing). Our $\mathcal{O}(N)$ algorithm reduces the time complexity of obtaining a solution from the core by as much as 71.67\% when compared with the \emph{Shapley value}.

==> related.tex <==
He et al. \cite{he2018s} study the allocation of edge resources to different applications by jointly considering request scheduling and service placement. The authors show that the problem is NP-hard and the complexity arises from the placement subproblem. They propose an approximation algorithm for homogeneous network settings and efficient heuristics for general network settings. 
Jia et al. \cite{jia2015optimal} discuss edge cloud placement and allocation of the resources to mobile users in the edge cloud in a Wireless Metropolitan Area Network (WMAN). They propose an algorithm that places edge clouds at user/application dense regions of the WMAN. Furthermore they also assign resources to users in the deployed edge clouds while balancing the workload among the edge clouds. Xu et al. \cite{xu2016efficient} discuss edge cloud placement in a large-scale WMAN which contains multiple wireless access points (APs). The goal of the placement problem is to minimize the average access delay between the users and the edge clouds. Our work differs from \cite{he2018s,jia2015optimal,xu2016efficient} as we are dealing with resource sharing and allocation in already existing edge clouds. 
 Our objective is to optimally utilize the available resources and allocate them to the applications. Rather than dealing with a single objective optimization problem, we deal with a multi-objective optimization setting where each edge cloud can have its own particular objective (latency, throughput, security etc.). We obtain Pareto optimal allocations and show that the grand coalition of all the edge clouds is stable where no edge cloud has any incentive to leave the coalition.  





